Strangeness and charm in quark-gluon hadronization

This dissertation presents a theoretical study of soft hadron production in relativistic heavy-ion collisions. We explore the principles governing the hadronization of the expanding QGP fireball, and to understand its properties. Much of the ongoing effort is to demonstrate the validity of a QGP hadronization model which describes the particle production data accurately. We begin with a centrality study of multistrange hadrons from Au-Au collisions at 62.4 GeV at RHIC. We show that the statistical hadronization model (SHM) well describes particle production in QGP hadronization. For all centralities, the physical properties are compatible with the earlier proposed critical hadronization pressure suggesting universal hadronization conditions of QGP. Heavy-ion collisions at LHC present a new challenge for SHM in describing particle production at TeV energy scales. We show that the chemical non-equilibrium model gives a good description of the hadron production in Pb--Pb collisions at 2.76 TeV consistently as a function of centrality. Moreover, the model parameters assume expected values suggested by previous studies at lower energies. The quark-gluon plasma fireball hadronizes at the same universal hadronization conditions, that is a common critical pressure, entropy and energy density. At LHC energies, a significant amount of charm is expected to be produced and it is therefore crucial to incorporate charm into the present description of particle production. We present an upgraded SHARE with CHARM program, that quantifies the effect of charm on the yield of lighter hadrons and physical properties of the hadronizing fireball. In addition to light flavors ($u,d,s$), SHARE with CHARM describes charm hadron production and decays. We observe, that according to present experimental results, charm decays mainly affect the yields of multistrange particles.

==> abstract.tex <==
This dissertation presents a theoretical study of soft hadron production in relativistic heavy-ion collisions. The aim is to explore the principles governing the hadronization of the expanding quark-gluon plasma (QGP) fireball, and to understand its properties. Strange hadron production and strangeness abundance in the QGP help us to look before the instant of hadronization. Consideration of entropy and charm production further enhances the reach back in time to the first instances of the heavy ion collision.

Much of the ongoing effort is to demonstrate the validity of a  QGP hadronization model which describes the particle production data accurately and thus allows us to carry out the above research program. We begin with performing a centrality dependent study of multistrange hadrons from Au--Au collisions at $\sqrt{s_{NN}}=62.4$~GeV, data obtained at the Relativistic Heavy Ion Collider (RHIC). We show that the statistical hadronization model (SHM) well describes particle production in QGP hadronization.  For all centralities, the particle production conditions are compatible with the earlier proposed critical hadronization pressure suggesting a set of universal hadronization conditions of QGP. 


Heavy-ion collisions at the Large Hadron Collider (LHC) present a new challenge for SHM in describing particle production at TeV energy scales. We show that the chemical non-equilibrium model gives a good description of the hadron production in Pb--Pb collisions at $\sqrt{s_{NN}}=2.76$~TeV not only in central collisions, where the equilibrium model struggled to describe the baryon to meson ratio, but consistently as a function of centrality. Moreover, the model parameters, such as chemical freeze--out temperature, assume expected values suggested by results from previous studies at lower energies. The quark-gluon plasma fireball hadronizes at the same universal hadronization conditions, that is a common critical pressure, entropy and energy density. 

At LHC energies, a significant amount of charm is expected to be produced in the initial hard parton scattering processes. It is therefore crucial to incorporate charm into the present description of particle production. We present a new tool, an upgraded SHARE with CHARM program, that quantifies the effect of charm on the yield of lighter hadrons and physical properties of the hadronizing fireball. In addition to light flavors ($u,d,s$), SHARE with CHARM describes charm hadron production and decays of charm hadrons. We observe, that according to present experimental results, charm decays mainly affect the yields of multistrange particles.


This dissertation begins with an introduction to the particle production in heavy-ion collisions and SHM framework, followed by a summary of results that are either published or submitted to peer-reviewed journals and others which are published as conference proceedings. Reprints of the publications are attached to the dissertation as appendices. Each appendix is prefaced with a short summary of presented results.

==> dedication.tex <==
\begin{center}
\emph{... to my parents, Ludmila and Petr Petran.}

\vspace{28 pt}

\emph{And also to you --- thanks for reading.}
\end{center}


